Monodromy Solver: Sequential and Parallel

We describe, study, and experiment with an algorithm for finding all solutions of systems of polynomial equations using homotopy continuation and monodromy. This algorithm follows a framework developed in previous work and can operate in the presence of a large number of failures of the homotopy continuation subroutine. We give special attention to parallelization and probabilistic analysis of a model adapted to parallelization and failures. Apart from theoretical results, we developed a simulator that allows us to run a large number of experiments without recomputing the outcomes of the continuation subroutine.

==> proofs.tex <==

\begin{proof}[Proof of Proposition~\ref{prop2}]
Note that we may assume $\head(t) = v$ for all  $t\in A$ by Remark~\ref{rem:only-v-matters}. 

Let $\Omega(Q,C,A)$ denote the set of possible idle states that could result from completing $A$. 
This forms a probability space, 
with the probability $p(x)$ for $x \in \Omega(Q,C,A)$ equal to the probability of reaching state $x$ by executing all tasks in $A$ under Assumption~\ref{randomAssumption}. 

To shorten the notation let $\#_v(x) = |Q'_v(x)|$. We note that
\begin{equation}\label{line1}
\E_v(Q,C,A\cup \{t\})=\sum_{x\in \Omega(Q,C,A\cup\{t\})} p(x) \#_v(x)
\end{equation}
by the definition of expected value.

% Define $\Delta\E_t(x):= \E(Q(x),C(x),A(x) \cup \{t\}) - \E(x)$. 
% Let $p(t|x)$ be the probability that $t$ finds a new
% solution in the case of state $x$ assuming $t$ is appended to $A(x)$ and {\bf executed first}.
% \marginpar{Note: I think you are using this only when $A(x)=\emptyset$. }

%\red{I don't whink $\Delta\E_t(x) = p(t|x)$. The most we can say is that one ``approximates'' the other in a certain sense. Also, $p(t|x)$ is bad notation: it looks like a conditional probability. Perhaps $p_t(x)$ (if we need a short one)?}
% \red{You're definitely right that $\Delta\E_t(x) \neq p(t|x)$---I was
% overzelous in trying to put things into the new notation. In my view, it {\em
% is} a conditional probability though, since it's the probability of $t$ finding
% a new solution given event $x$. Maybe that's wrong though?}

Let $t=(s,\ar e)$.
For a state $x$ such that $A(x)=\emptyset$, let $p(t|x)$ be the probability
that $t$ finds a new solution in the case of $x$. In other words,
$$
p(t|x) = \E(Q(x),C(x),\{t\})-\E(Q(x),C(x),\emptyset) = \begin{cases}
\frac{d-|Q_{\head(t)}|}{d-|C_e(x)|}, & s\notin Q_{\tail(t)}(x);\\
0,&\text{otherwise}.
\end{cases}
$$
Now note that each possible state $x\in
\Omega(Q,C,A\cup\{t\})$ can be broken up into a state resulting from $A$ with
two possibilities for $t$, namely $t$ finding or failing to find a new solution.
We can therefore rewrite (\ref{line1}) as
\def\sumIndices{\mathclap{\substack{x\in \Omega(Q,C,A)}}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "art"
%%% End:

